Translating predictive distributions into informative priors

When complex Bayesian models exhibit implausible behaviour, one solution is to assemble available information into an informative prior. Challenges arise as prior information is often only available for the observable quantity, or some model-derived marginal quantity, rather than directly pertaining to the (usually latent) parameters in our model. We propose a method for translating available prior information, in the form of an elicited distribution for the observable or model-derived marginal quantity, into an informative joint prior. Our approach proceeds given a parametric class of prior distributions with as yet undetermined hyperparameters, and minimises the difference between the supplied elicited distribution and corresponding prior predictive distribution. We employ a global, multi-stage Bayesian optimisation procedure to locate optimal values for the hyperparameters. Three examples illustrate our approach: a cure-fraction survival model, where censoring implies that the observable quantity is _a priori_ a mixed discrete/continuous quantity; a setting in which prior information pertains to $R^{2}$ -- a model-derived quantity; and a nonlinear regression model.

==> tex-input/0081-repulsiveness-objective.tex <==
\begin{equation}
  \tilde{R}(\lambda) = \sum_{1 \leq l < l' \leq L} 
  - \log \left( 
    1 - \exp\left\{-c_{0} \| \lambda_{l} - \lambda_{l'}\|_{2}\right\}
  \right),
  \label{eqn:repulsiveness-objective}
\end{equation}

==> tex-input/pbbo-methodology/0011-theoretical-discrep-definition-population.tex <==
\begin{equation}
  \lambda^{*} =
    \min_{\lambda \in \Lambda} \tilde{D}^{\text{pop}}(\lambda) =
    \min_{\lambda \in \Lambda} \int_{\mathcal{Y}} d(\Pd(Y \mid \lambda), \tc(Y)) \text{d}Y
  \label{eqn:theoretical-discrep-definition-population}
\end{equation}

==> tex-input/pbbo-methodology/0014-theoretical-discrep-definition-covariate-importance.tex <==
\begin{equation}
  \tilde{D}(\lambda \mid \boldsymbol{X}) =
    \frac{1}{R}
    \sum_{r = 1}^{R}
    \int d(
      \Pd(Y \mid \lambda, X_{r}),
      \tc(Y \mid X_{r})
    )
    \frac {
      \text{d}\tc(Y \mid X_{r})
    } {
     \text{d}\Q(Y \mid X_{r})
    }
    \text{d}\Q(Y \mid X_{r}).
  \label{eqn:theoretical-discrep-definition-covariate-importance}
\end{equation}

==> tex-input/pbbo-methodology/0021-importance-discrepancy-population-definition.tex <==
\begin{equation}
  \log(D^{\text{pop}}(\lambda)) =
    -\log(I) +
    \log\left(
      \sum_{i = 1}^{I}
      \exp\left\{
        z(u_{i})
      \right\}
    \right),
  \label{eqn:importance-discrepancy-population-definition}
\end{equation}


==> tex-input/pbbo-methodology/0061-crs2-full-algorithm.tex <==
\begin{algorithm}[H]
  \caption{Controlled random search 2 \citep{price_global_1983} with local mutation \citep{kaelo_variants_2006} for minimising the deterministic function $f$.}
    \label{alg:crs2-full-algorithm}
  \begin{algorithmic}[1]
    \Require{Objective function $f(\lambda)$ (to be minimised), feasible region or support $\Lambda \subseteq \mathbb{R}^{n}$, population size $N$}
    \Statex
    \Function{CRS2 with local mutation}{$N$}
      \State Generate $N \gg n$ initial points $\mathcal{A} = \{\lambda_{i}\}_{i = 1}^{N}$ from a space filling design covering $\Lambda$
      \State Evaluate $f$ at each $\lambda \in \mathcal{A}$ storing the result such that $\mathcal{A} = \{\lambda_{i}, f(\lambda_{i})\}_{i = 1}^{N}$
      \State Sort $\mathcal{A}$ by $f(\lambda_{i})$ so that $\lambda_{1}$ is the current best value (i.e. lowest) $f(\lambda_{1})$ and $\lambda_{N}$ the worst (i.e highest) $f(\lambda_{N})$
      \While{Not converged}
        \State Sample without replacement $n$ values of $\lambda$ uniformly at random from $\mathcal{A} ~ \smallsetminus ~ \{\lambda_{1}, ~ f(\lambda_{1})\}$ and store them in $\mathcal{B} = \{\lambda_{j}\}_{j = 2}^{n + 1}$
        \State Add the current best value $\lambda_{1}$ and $f(\lambda_{1})$ to $\mathcal{B}$
        \State Compute the centroid (coordinate-wise mean) $\hat{C} = \frac{1}{n}\sum_{j = 1}^{n} \lambda_{j}$ using $n$ of the $n + 1$ points in $\mathcal{B}$
        \State Compute the \emph{trial point} $\tilde{\lambda} = 2 \hat{C} - \lambda_{n + 1}$, for $\lambda_{n + 1} \in \mathcal{B}$, and evaluate $f(\tilde{\lambda})$
        \If{$f(\tilde{\lambda}) < f(\lambda_{N})$}
          \State Remove $\{\lambda_{N}, f(\lambda_{N})\}$ from $\mathcal{A}$ 
          \State Insert $\{\tilde{\lambda}, f(\tilde{\lambda})\}$ appropriately so that $\mathcal{A}$ remains sorted
        \Else \Comment{\textit{Local mutation from \citet{kaelo_variants_2006}}}
          \State Sample $\omega$ from the $n$-dimensional uniform distribution $\text{Unif}[0, 1]^{n}$
          \State Compute new \emph{trial point} $\tilde{\lambda}^{\text{LM}} = (1 + \omega)\lambda_{1} - \omega\tilde{\lambda}$ and evaluate $f(\tilde{\lambda}^{\text{LM}})$
          \If{$f(\tilde{\lambda}^{\text{LM}}) < f(\lambda_{N})$}
            \State Remove $\{\lambda_{N}, f(\lambda_{N})\}$ from $\mathcal{A}$
            \State Insert $\{\tilde{\lambda}^{\text{LM}}, f(\tilde{\lambda}^{\text{LM}})\}$ appropriately so that $\mathcal{A}$ remains sorted
          \EndIf
        \EndIf
        \State Check convergence criteria: if $\lvert \lambda_{1} - \lambda_{N}\rvert < 10^{-6}$ then \textbf{break}
      \EndWhile
      \State \textbf{return:} $\lambda^{*} = \lambda_{1}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

%$\kappa$, $N(\lambda)$, $N_{\text{CRS2}}$, $N_{\text{BO}}$, $N_{\text{batch}}$,

% bayes opt batch algorithm
% batch to design for next batch algorithm
% pbbo algorithm

==> tex-input/pre.tex <==
\usepackage{amsmath,amssymb,mathtools,bbm}
% I always seem to need tikz for something
\usepackage{tikz}
\usetikzlibrary{positioning, shapes, intersections, through, backgrounds, fit, decorations.pathmorphing}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{setspace}
\onehalfspacing

% \usepackage{lineno}
% % \linenumbers

% \usepackage{xr}
% \makeatletter
% \newcommand*{\addFileDependency}[1]{% argument=file name and extension
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{%
%     \externaldocument{#1}%
%     \addFileDependency{#1.tex}%
%     \addFileDependency{#1.aux}%
% }

% \myexternaldocument{priors-by-optimisation-supplement}

% required for landscape pages. beware, they make build times very long.
\usepackage{pdflscape}
\usepackage{placeins}

% table - `gt' package uses these, often unimportant
%\usepackage{longtable}
\usepackage{booktabs}
%\usepackage{caption}
\usepackage{colortbl}

\usepackage{color}
\definecolor{myredhighlight}{RGB}{180, 15, 32}
\definecolor{mydarkblue}{RGB}{0, 33, 79}
\definecolor{mymidblue}{RGB}{44, 127, 184}
\definecolor{mylightblue}{RGB}{166, 233, 255}
\definecolor{mywhwlow}{RGB}{234, 164, 99}

\usepackage{accents}
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}

\setcounter{secnumdepth}{3}

% \renewcommand{\floatpagefraction}{0.8}
% \renewcommand{\topfraction}{0.8}
% \renewcommand{\bottomfraction}{0.8}
% \renewcommand{\textfraction}{0.25}

% pd stands for: probability distribution and is useful to distringuish
% marignals for probabilities specifically p(p_{1}) and the like.
\newcommand{\pd}{\text{p}}
\newcommand{\Pd}{\text{P}}
\newcommand{\q}{\text{q}}
\newcommand{\Q}{\text{Q}}
\newcommand{\w}{\text{w}}
\newcommand{\pdr}{\text{r}}
\newcommand{\pdrh}{\hat{\text{r}}}

% pbbo stuff
\newcommand{\tc}{\text{T}}
\newcommand{\tp}{\text{t}}

% melding
\newcommand{\ppoolphi}{\pd_{\text{pool}}(\phi)}
\newcommand{\ppool}{\pd_{\text{pool}}}
\newcommand{\pmeld}{\pd_{\text{meld}}}

% the q(x)w(x), "weighted target" density 
% for the moment I'm going to call it s(x), as that is the next letter of the 
% alphabet. Can change it later
\newcommand{\s}{\text{s}}
% direct density estimate - replaces lambda.
\newcommand{\ddest}{\text{s}}
% target weighting function
\newcommand{\tarw}{\text{u}}

% constants - usually sizes of things
\newcommand{\Nx}{N}
\newcommand{\Nnu}{\text{N}_{\text{nu}}}
\newcommand{\Nde}{\text{N}_{\text{de}}}
\newcommand{\Nmc}{\text{N}_{\text{mc}}}
\newcommand{\Nw}{W}
\newcommand{\Nm}{M}
\newcommand{\Ns}{S}

% locales - could switch to x and x'
\newcommand{\xnu}{x_{\text{nu}}}
\newcommand{\xde}{x_{\text{de}}}
\newcommand{\phinu}{\phi_{\text{nu}}}
\newcommand{\phide}{\phi_{\text{de}}}

% sugiyama stuff
\newcommand{\pdnu}{\pd_{\text{nu}}}
\newcommand{\pdde}{\pd_{\text{de}}}

% indices 
\newcommand{\wfindex}{w}
\newcommand{\sampleindex}{n}
\newcommand{\modelindex}{m}
\newcommand{\stageindex}{s}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}
\newcommand{\kldiv}{\text{KL}\infdivx}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\newcommand{\lse}{\text{logSumExp}}

\newcommand*\Let[2]{\State #1 $\gets$ #2}
\algrenewcommand\alglinenumber[1]{
    {\sf\footnotesize\color{lightgray}#1}}
\algrenewcommand\algorithmicrequire{\textbf{Inputs:}}
\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}

\def\dodoi#1{doi: \href{https://doi.org/#1}{\nolinkurl{#1}}}
\def\dourl#1{\href{http://#1}{\nolinkurl{#1}}}

==> tex-input/r2-examples/0011-gaussian-prior-def.tex <==
\begin{equation}
  \beta_{j} \sim \text{N}\left(0, \frac{\sigma^{2}}{\gamma}\right).
  \label{eqn:gaussian-prior-def}
\end{equation}

==> tex-input/r2-examples/0012-dirichlet-laplace-definition.tex <==
\begin{equation}
  \beta_{j} \sim \text{Laplace}\left(0, \sigma \phi_{j} \tau \right), \quad
  (\phi_{1}, \ldots, \phi_{p}) \sim \text{Dirichlet}(\alpha, \ldots, \alpha), \quad
  \tau \sim \text{Gamma}(p \alpha, 1 \mathop{/} 2).
  \label{eqn:bhattacharya_dirichletlaplace_2015}
\end{equation}

==> tex-input/surv-example/0012-surv-prior-dists.tex <==
\begin{equation}
  \begin{gathered}
  \pi \sim \text{Beta}(a_{\pi}, b_{\pi}), \quad
  \gamma \sim \text{Gamma}(\alpha, \beta), \\
  \beta_{0} \sim \text{Normal}(\mu_{0}, \sigma_{0}^{2}), \quad
  \boldsymbol{\beta} \sim \text{MVSkewNormal}(\boldsymbol{0}, \boldsymbol{S}, \boldsymbol{\eta}).
  \end{gathered}
  \label{eqn:surv-prior-dists}
\end{equation}
